Zero-shot Visual Commonsense Immorality Prediction

Artificial intelligence is currently powering diverse real-world applications. These applications have shown promising performance, but raise complicated ethical issues, i.e. how to embed ethics to make AI applications behave morally. One way toward moral AI systems is by imitating human prosocial behavior and encouraging some form of good behavior in systems. However, learning such normative ethics (especially from images) is challenging mainly due to a lack of data and labeling complexity. Here, we propose a model that predicts visual commonsense immorality in a zero-shot manner. We train our model with an ETHICS dataset (a pair of text and morality annotation) via a CLIP-based image-text joint embedding. In a testing phase, the immorality of an unseen image is predicted. We evaluate our model with existing moral/immoral image datasets and show fair prediction performance consistent with human intuitions. Further, we create a visual commonsense immorality benchmark with more general and extensive immoral visual contents. Codes and dataset are available at https://github.com/ku-vai/Zero-shot-Visual-Commonsense-Immorality-Prediction. Note that this paper might contain images and descriptions that are offensive in nature.

==> src/commonsense_morality.tex <==
Immoral image should be predicted for a wide range of situations from the model in order to assist individuals to create the same annotation repeatedly for the restriction of the video content ranking system or the evidence of the criminal situation. Furthermore, predicted immorality should be accepted by a staggering number of people considering all the diverse backgrounds and ethnic groups. Because of the ambiguous ground truths, the large scale of user research is vital for testing. Nevertheless, the ETHICS commonsense morality dataset, which was made with general consensus of morality in natural language, has already gone through this process and obtained agreement rate over 0.9 with the final dataset’s labels from the US. The definition of commonsense immorality is first-person character clearly should not have done that action. It is able to cover all the various immoral behaviors like violation of the law or unconscionable behavior. In this context, our research may utilize the information of commonsense immorality from the ETHICS commonsense morality dataset, which demonstrates the process of shifting the natural language domain to visual domain.


==> src/tables/table-dataset-comparison.tex <==
% original table
% {
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.3} 
% \begin{table}[t]
%     \caption{Comparison between existing immoral image datasets and our created visual commonsense immorality dataset.}
%     \label{tab:datasets}
% 	\begin{center}
%     	\resizebox{.8\linewidth}{!}
%     	{%
%     	\begin{tabular}{@{}lrrr@{}} \toprule
%     	    % 전체 Image를 비교할 경우 SMID가 더 많아 'Immoral Image' 기준으로 비교
%     	    Dataset & \# of Immoral Images & Content & \# of Immoral types\\\midrule
%     	    Socio-Moral Image~\cite{SMID} & 962 & labeled photographic images & - \\
%     	    Sexual Intent Detection~\cite{ganguly2017sexual} & 466 & sexuality & 2\\
%     	    Real Life Violence Situations~\cite{soliman2019violence}& 1,000 & violence & 2\\
%     	    NSFW~\cite{nsfw} & 16,103 & sexuality & 5\\\midrule
%     	    Visual Commonsense Immorality (ours) & 2,172 & felony, anti-social, environment & 25 \\\bottomrule
%         \end{tabular}}
%      \end{center}
%      \vspace{-1.5em}
% \end{table}
% }


% \begin{table}
% 	\begin{minipage}{0.55\linewidth}
% 	\caption{Comparison between existing immoral image datasets and our created visual commonsense immorality dataset.}
% 	\vspace{1em}
% 		\label{tab:le}
% 		\centering
% 		\resizebox{\textwidth}{!}
% 		{
% 		\begin{tabular}{@{}lrr@{}} \toprule
%     	     & \# of  & \\
%     	    Dataset &Immoral Images(types) &  Content\\\midrule
%     	    Socio-Moral Image~\cite{SMID} & 962(-) & labeled photographic images \\
%     	    Sexual Intent Detection~\cite{ganguly2017sexual} & 466(2) & sexuality\\
%     	    Real Life Violence Situations~\cite{soliman2019violence}& 1,000(2) & violence\\
%     	    NSFW~\cite{nsfw} & 16,103(5) & sexuality\\\midrule
%     	    Visual Commonsense Immorality (ours) & 2,172(25) & felony, anti-social, environment \\\bottomrule
%         \end{tabular}}
% 	\end{minipage}\hfill\hspace{-1.5em}
% 	\begin{minipage}{0.55\linewidth}
% 		\centering
% 		\captionof{figure}{Different types of examples}
% 		\vspace{1em}
% 		\label{figu:re}
% 		\includegraphics[width=0.8\textwidth]{images/without-eps-converted-to.eps}
% % 		\includegraphics[width=0.8\textwidth]{images/with_nsfw.eps}
% 	\end{minipage}
% 	\vspace{-1.5em}
% \end{table}

  
  
%Our dataset consists of general and explicit content in terms of immorality. 25 keywords (e.g. armed robbery, secondhand smoking, fly-tipping, etc) are based on 3 categories: felony, anti-social, and environment.
